A Spectral Condition for Feature Learning

The push to train ever larger neural networks has motivated the study of initialization and training at large network width. A key challenge is to scale training so that a network's internal representations evolve nontrivially at all widths, a process known as feature learning. Here, we show that feature learning is achieved by scaling the spectral norm of weight matrices and their updates like $\sqrt{\texttt{fan-out}/\texttt{fan-in}}$, in contrast to widely used but heuristic scalings based on Frobenius norm and entry size. Our spectral scaling analysis also leads to an elementary derivation of \emph{maximal update parametrization}. All in all, we aim to provide the reader with a solid conceptual understanding of feature learning in neural networks.

==> algorithm/frobenius.tex <==
\begin{algorithm}[H]
\caption{Frobenius-muP. Implementation of Condition \ref{def:convert} via Frobenius normalization.}
   \label{alg:frobenius}
\begin{minipage}[t]{.5\textwidth}
\begin{algorithmic}
    \STATE \COMMENT{Initialization}
   \FOR{{\bfseries layer $\ell$ in $\{1,2,...,L\}$}}
   \STATE sample $(\mW_\ell)_{ij} \overset{\mathrm{iid}}{\sim} \normal(0,1)$
   \STATE rescale $\mW_\ell \gets \frac{\mW_\ell}{\norm{\mW_\ell}_F / \sqrt{\min(d_\ell,d_{\ell-1})}} \cdot \sqrt{\frac{d_\ell}{d_{\ell-1}}}$
   \ENDFOR
\end{algorithmic}
\end{minipage}
\begin{minipage}[t]{.5\textwidth}
\begin{algorithmic}
   \STATE \COMMENT{Weight update}
   \FOR{{\bfseries layer $\ell$ in $\{1,2,...,L\}$}}
   \STATE update $\mW_\ell \gets \mW_\ell - \eta\cdot  \frac{\nabla_{\mW_\ell}\mathcal{L}}{\norm{\nabla_{\mW_\ell}\mathcal{L}}_F} \cdot \sqrt{\frac{d_\ell}{d_{\ell-1}}}$
   \ENDFOR
\end{algorithmic}
\end{minipage}
\end{algorithm}

==> algorithm/mup.tex <==
\begin{algorithm}[H]
\caption{Vanilla-muP. Implementation of Condition \ref{def:convert} via norm estimates.}
   \label{alg:mup}
\begin{minipage}[t]{.5\textwidth}
\begin{algorithmic}
    \STATE \COMMENT{Initialization}
   \FOR{{\bfseries layer $\ell$ in $\{1,2,...,L\}$}}
   \STATE sample $(\mW_\ell)_{ij} \overset{\mathrm{iid}}{\sim} \normal(0,1)$
   \STATE rescale $\mW_\ell \gets \frac{\mW_\ell}{\sqrt{d_\ell d_{\ell-1}} / \sqrt{\min(d_\ell,d_{\ell-1})}} \cdot \sqrt{\frac{d_\ell}{d_{\ell-1}}}$
   \ENDFOR
\end{algorithmic}
\end{minipage}
\begin{minipage}[t]{.5\textwidth}
\begin{algorithmic}
   \STATE \COMMENT{Weight update}
   \FOR{{\bfseries layer $\ell$ in $\{1,2,...,L\}$}}
   \STATE update $\mW_\ell \gets \mW_\ell - \eta\cdot  \frac{\nabla_{\mW_\ell}\mathcal{L}}{\sqrt{d_{\ell-1} / d_\ell}} \cdot \sqrt{\frac{d_\ell}{d_{\ell-1}}}$
   \ENDFOR
\end{algorithmic}
\end{minipage}
\end{algorithm}

==> algorithm/spectral.tex <==
\begin{algorithm}[H]
\caption{Spectral-muP. Implementation of Condition \ref{def:convert} via spectral normalization.}
   \label{alg:spectral}
\begin{minipage}[t]{.5\textwidth}
\begin{algorithmic}
    \STATE \COMMENT{Initialization}
   \FOR{{\bfseries layer $\ell$ in $\{1,2,...,L\}$}}
   \STATE sample $(\mW_\ell)_{ij} \overset{\mathrm{iid}}{\sim} \normal(0,1)$
   \STATE rescale $\mW_\ell \gets \frac{\mW_\ell}{\norm{\mW_\ell}_*} \cdot \sqrt{\frac{d_\ell}{d_{\ell-1}}}$
   \ENDFOR
\end{algorithmic}
\end{minipage}
\begin{minipage}[t]{.5\textwidth}
\begin{algorithmic}
   \STATE \COMMENT{Weight update}
   \FOR{{\bfseries layer $\ell$ in $\{1,2,...,L\}$}}
   \STATE update $\mW_\ell \gets \mW_\ell - \eta\cdot  \frac{\nabla_{\mW_\ell}\mathcal{L}}{\norm{\nabla_{\mW_\ell}\mathcal{L}}_*} \cdot \sqrt{\frac{d_\ell}{d_{\ell-1}}}$
   \ENDFOR
\end{algorithmic}
\end{minipage}
\end{algorithm}

==> apps/picture_w_nonlin.tex <==
\section{A spectral picture of feature learning (with nonlinearities)}
\label{app:heuristic_picture_w_nonlin}

\jamie{Jamie to write}

==> old_sections/comparison_to_other_scalings.tex <==
\section{Comparison to common scalings}
% \label{sec:redacted}

Here we show that our spectral scaling --- which we have now shown to be the unique choice giving feature learning at large width --- is equivalent to muP.
We also apply our spectral lens to other common parameterizations and illuminate how they fail to learn features as a result of their last-layer scalings.

Our task is made nontrivial by the fact that virtually all other works discussing neural network parameterizations work with a different set of variables --- namely, parameterwise init scales $\sigma_\ell$ and layerwise learning rates $\eta_\ell$ --- whereas we work in terms of $\norm{\mW_\ell^0}_*$ and $\norm{\Delta \mW_\ell}_*$.
Of course, this is the point: these spectral quantities provide a cleaner language more suitable for analysis of forward and backward dynamics in sequential tensor operations.
We can convert between these sets of quantities without much trouble.

Recalling from Section \ref{subsec:important_norms} that $\norm{\mW_\ell^0} \sim \sigma_\ell \max( \sqrt{d_\ell}, \sqrt{d_{\ell-1}})$, we find that Condition \ref{cond:scaling} implies that
\begin{equation} \label{eqn:sigma_scaling}
    \sigma_\ell \sim \min \left( \frac{1}{\sqrt{d_{\ell-1}}}, \frac{\sqrt{d_\ell}}{d_{\ell-1}} \right).
\end{equation}
To find the scalings for learning rate, recall from Section \ref{sec:heuristic_picture} that $\Delta \mW_\ell = -\eta_\ell \vg_\ell \vh_{\ell-1}\T$ with $\vg_\ell = \nabla_{\vh_\ell} \L$.
We expect that $\Theta(1)$ updates to the output elements will cause a $\Theta(1)$ decrease in the loss, and thus $\norm{\vg_L}_2 \sim \frac{1}{\sqrt{d_L}}$.%
\footnote{Note that, since $d_L = \Theta(1)$ by assumption, all that really matters is that $\norm{\vg_L}_2 = \Theta(1)$.}
Assuming maximal action on the backward pass, we have that $\norm{\vg_\ell}_2 \sim \frac{1}{\sqrt{d_\ell}}$.
Enforcing that $\norm{ \Delta \mW_\ell }_* \sim \sqrt{d_\ell / d_{\ell-1}}$ implies that
\begin{equation} \label{eqn:eta_scaling}
    \eta_\ell
    % \sim \frac{\sqrt{d_\ell}}{\sqrt{d_{\ell-1}}} \frac{1}{\norm{\vg_\ell}_2 \norm{\vh_{\ell-1}}_2}
    \sim \frac{d_\ell}{d_{\ell-1}}.
\end{equation}

\subsection{Our spectral scaling is equivalent to muP}

Comparing with the hyperparameter tables in [muP CITATIONS], we see that Equations \ref{eqn:sigma_scaling} and \ref{eqn:eta_scaling} are equivalent to muP.
\jamie{Greg, can you say more here? Do we also recover the scalings for convnets + transformers?}

While it is possible to derive muP working in terms of $\{(\sigma_\ell$, $\eta_\ell)\}_\ell$, such a derivation is fairly cumbersome.
Our spectral approach gives a clean derivation because it provides a natural language for the discussion of tensor alignment, which the parameterwise approach does not.
As additional evidence that the spectral perspective is the right one, note that Equations \ref{eqn:sigma_scaling} and \ref{eqn:eta_scaling} give general formulae valid at all layers, whereas prior analyses taking a parameterwise view instead give ad-hoc scalings for each layer.

\subsection{Comparison to the neural tangent parameterization}

Many theoretical studies of wide neural networks use the ``neural tangent parameterization" (NTP) in which neural network training is effectively linear in its parameters [CITATIONS].
How does the NTP differ from muP?
The key difference is that the NTP prescribes
\begin{equation} \label{eqn:ntp_sigma_scaling}
    \sigma_\ell \sim \frac{1}{\sqrt{d_{\ell-1}}},
\end{equation}
which differs from Equation \ref{eqn:sigma_scaling} in layers with $\texttt{[fan-in]} \gg \texttt{[fan-out]}$, namely the final layer.
As a result, \textit{the spectral norm of the last layer is too large to allow feature learning earlier in the network}: if $\norm{\Delta \vh_{L-1}}_2 \sim \sqrt{d_{L-1}}$ (as per D3), then $\norm{\Delta \vh_L}_2 \sim \sqrt{d_{L-1} d_L}$ will be too large.

Using standard statistics of sums of \textit{i.i.d.} variables, we find that after parameterwise initialization using Equation \ref{eqn:ntp_sigma_scaling},
it is easily shown that $\norm{\vg_\ell}_2 = \norm{(\mW_\ell^0)\T \vg_{\ell+1}}_2 \sim \norm{\vg_{\ell+1}}_2$ for all $\ell$.
It follows that
\begin{equation}
    \norm{\vg_\ell}_2 \sim \norm{\vg_{L}}_2 \sim \frac{1}{\sqrt{d_L}}
\end{equation}
for all $\ell$.
To effect an order-one change in the loss, an update to $\mW_\ell$ must satisfy
\begin{equation}
    \Delta \L \sim \vg_\ell\T \Delta \vh_\ell
    = \norm{\vg_\ell}_2 \norm{\Delta \vh_\ell}_2
    = \norm{\vg_\ell}_2 \norm{\Delta \mW_\ell}_* \norm{\vh_{\ell-1}}_2
    \sim \frac{\sqrt{d_{\ell-1}}}{\sqrt{d_L}} \norm{\Delta \mW_\ell}_*
    \sim 1
\end{equation}
and thus
$\norm{\Delta \vh_\ell}_2 \sim \sqrt{d_{L}}$
and
$\norm{\Delta \mW_\ell}_* \sim \sqrt{d_L / d_{\ell-1}}$.
From the fact that $\Delta \mW_\ell = - \eta_\ell \vg_\ell \vh_{\ell-1}\T$, we recover we recover the NTP learning rate scaling $\eta_\ell \sim 1 / d_{\ell-1}$.
\jamie{put this in a footnote?}

We thus conclude that
\begin{equation}
    \norm{\Delta \vh_\ell}_2 \ll \norm{\vh_\ell^0}_2
    \ \ \ \ \
    \text{and}
    \ \ \ \ \
    \norm{\Delta \mW_\ell}_* \ll \norm{\mW_\ell^0}_*.
\end{equation}
This states, in spectral terms, that \textit{the updates are dominated by the initialization}.
This implies that the NTP does not learn features and that its weight tensors do not align.
Our spectral view shows that these shortcomings are in fact two sides of the same coin.

\subsection{Comparison to the standard parameterization}

What about the ``PyTorch standard" parameterization (SP) suggested by classic works [CITATIONS]?
These works use the same initialization as the NTP, and so the SP is similarly doomed.
However, the SP actually has an \textit{additional} problem: it typically assumes a constant learning rate
\begin{equation}
    \eta_\ell \sim 1
\end{equation}
or at least one which is the same across layers ($\eta_\ell \sim \eta_{\ell'}$).
A $\Theta(1)$ learning rate will cause blowup when training the last layer, and our analysis of the NTP showed that different layers need different learning rates in order to each act at the proper order.
The best choice is
\begin{equation}
    \eta_\ell = \frac{1}{\sqrt{\max\limits_{\ell' \le L-1} d_{\ell'}}},
\end{equation}
which recovers the NTP scaling at the widest layers and gives trivial, sub-leading-order updates at all others.
Because the SP is strictly worse than the NTP, we will generally not discuss it elsewhere in this paper.

==> old_sections/derivation.tex <==
\section{Unique derivation of spectral scalings from a single gradient step}
\label{sec:derivation}

We now examine the process by which weight tensors align early in training.
The result will be a clean derivation which identifies our spectral scalings as the unique set satisfying D1-D4.

\subsection{Alignment at initialization}
Suppose for simplicity that all hidden layers have the same width ($d_1 = d_2 = \cdots = d_{L-1} \gg d_0, d_L$).
We denote by $\mW_\ell^0$ the weights at layer $\ell$ upon random initialization.

Recalling from Section \ref{subsec:random_matrix_alignment} that random matrices act maximally on typical vectors unless they have $\texttt{[fan-out]} \ll \texttt{[fan-in]}$, we may make a key observation: \textit{all layers except the last one act maximally at init during the forward pass}.
The last layer is misaligned as\footnote{Note that $\Theta(\sqrt{1 / d_{L-1}})$ is the expected alignment of two random vectors.}
\begin{equation}
    \alignment(\mW^0_L, \vh_L) = \Theta(\sqrt{d_L / d_{L-1}}).
\end{equation}
Considering the backward pass (and so flipping \texttt{[fan-out]} and \texttt{[fan-in]}), we find the remarkable fact that \textit{all layers act maximally during the backward pass} except for $\mW_1^0$, through which we do not backpropagate anyways.
Because the readout layer $\mW_L^0$ acts maximally backwards, it will act maximally forwards on the updated forward signal when any earlier layer is updated --- that is,
\begin{equation}
    \alignment(\mW^0_L, \Delta \vh_{L-1}) = \Theta(1).
\end{equation}
This follows from the identities $\alignment(\mW^0_L, \vg_{L-1}) = \Theta(1)$ (due to Proposition \ref{prop:align_properties}(d)) and $\alignment(\vg_{L-1}\T, \Delta \vh_{L-1}) = \Theta(1)$ (due to Corollary \ref{cor:update-grad-align}).

\subsection{Derivation}

We are now ready to use our desiderata.
In light of the maximality of all but the final layer, achieving the hidden vector scaling mandated by D1 requires that
\begin{equation}
    {\color{blue}
        \norm{\mW_\ell^0}_* = \Theta \left( \sqrt{\frac{d_\ell}{d_{\ell-1}}} \right)
        \ \ \ \ \ \text{for} \ \ \ \ \
        \ell = 1 \ldots L \! - \! 1.
    }
\end{equation}
This is precisely the usual LeCun initialization.
Furthermore, because updates to tensors act maximally, satisfying the requirement of feature learning in D3 requires that
% $\norm{\Delta \mW_\ell}_*= \Theta \left( \sqrt{\frac{d_\ell}{d_{\ell-1}}} \right)$ for $\ell = 1 \ldots L \! - \! 1$.
\begin{equation}
    {\color{blue}
        \norm{\Delta \mW_\ell}_*= \Theta \left( \sqrt{\frac{d_\ell}{d_{\ell-1}}} \right)
        \ \ \ \ \
        \text{for}
        \ \ \ \ \
        \ell = 1 \ldots L \! - \! 1.
    }
\end{equation}
Any alternative would give $\norm{\Delta \vh_\ell}_2$ too big or too small.

We now examine the last layer.
Because $\mW^0_L$ acts maximally on $\Delta \vh_L$, we have that 
\begin{equation} \label{eqn:last_layer_maximal_step}
    \norm{\Delta \vh_L}_2
    = \norm{\mW^0_L \Delta \vh_{L-1}}_2
    \sim \norm{\mW^0_L}_* \norm{\Delta \vh_{L-1}}_2.
\end{equation}
Enforcing that $\norm{\Delta \vh_{L-1}}_2 = \Theta(\sqrt{d_{L-1}})$ from D3 and that $\norm{\Delta \vh_{L}}_2 = \Theta(\sqrt{d_{L}})$ from D4, we conclude from Equation \ref{eqn:last_layer_maximal_step} that
\begin{equation}
    {\color{blue}
        \norm{\mW^0_L}_* = \Theta \left( \sqrt{\frac{d_L}{d_{L-1}}} \right).
    }
\end{equation}
Finally, because updates act maximally, we see that taking a gradient step at layer $L$ gives
\begin{equation}
        \norm{\Delta \vh_L}_2 = \norm{\Delta \mW^0_L \vh_{L-1}}_2 \sim \norm{\Delta \mW^0_L}_* \norm{\vh_{L-1}}_2
\end{equation}
and thus enforcing D1 and D4 yields that
\begin{equation}
    {\color{blue}
        \norm{\Delta \mW_L}_*= \Theta \left( \sqrt{\frac{d_L}{d_{L-1}}} \right).
    }
\end{equation}
The four equations in {\color{blue}blue} constitute the spectral scaling of Condition \ref{cond:scaling} as desired.
This completes the derivation.

\subsection{All weight matrices are aligned after one step}

Only the final layer weight matrix was misaligned at initialization, and after the first gradient step on a particular example the updated weight matrix $\mW_L = \mW_L^0 + \Delta \mW_L$ will now act maximally.
Gradient descent thus puts the network in a fully maximal state, justifying Assumption \ref{assumption:full_maximality} in our heuristic picture of feature learning.

==> old_sections/desiderata.tex <==
\section{Desiderata for feature learning}
\label{sec:desiderata}

We want neural networks to retain proper feature learning at large width.
How do we make this requirement precise?
Here we state conditions which capture this notion:

\jamie{I was torn here about whether to phrase things in terms of vector norms (i.e. $\norm{\vh_\ell}_2 \sim d_\ell$) or in terms of element sizes. Vector norms would be nice because it is the language of the rest of the paper... I'll go with that for now.}

Consider a depth-$L$ neural network with layer sizes $\{d_\ell\}_{\ell = 0}^L$, in which layer $0$ is the input and layer $L$ is the output.
Let $\{\vh_\ell(\vx)\}_{\ell=1}^L$ be the network's layerwise representations, found via partial evaluation of the network on an input $\vx$ up to layer $\ell$, with $\vh_L(\vx)$ the network output.%
\footnote{These desiderata apply to any architecture, letting $d_\ell$ be the number of elements in $\vh_\ell$ (for example, $d_\ell = \mathtt{[width_\ell]} \times \mathtt{[height_\ell]} \times \mathtt{[channels_\ell]}$ for a convolutional layer). For structured architectures, replace $\norm{\vh_\ell(\vx)}_2$ with $\norm{\vh_\ell(\vx)}_F$ in the desiderata. \jamie{Is this helpful to say? We have a lot of footnotes here.}}
We want our network to satisfy the following \textit{four desiderata}:

\begin{enumerate}[leftmargin=1.2cm,itemsep=0pt,topsep=0pt,label=\textbf{\textlangle D\arabic*\textrangle}]
\item
At initialization, $\norm{\vh_\ell(\vx)}_2 = \Theta(\sqrt{d_\ell})$ for $\ell = 1 \ldots L-1$.
\label{d:hidden_init}
\item At initialization, $\norm{\vh_L(\vx)}_2 = \O(\sqrt{d_L})$.
\label{d:output_init}
\item
Performing a gradient step at layer $\ell$ must induce updates $\norm{\Delta \vh_\ell(\vx)} = \Theta(\sqrt{d_\ell})$ for $\ell = \ell \ldots L-1$ at all subsequent hidden layers.
\label{d:hidden_update}
\item
Performing a gradient step at layer $\ell$ must induce an update $\norm{\Delta \vh_L(\vx)} = \Theta(\sqrt{d_L})$ at the output.
\label{d:output_update}
\end{enumerate}

D1 follows from the fact that most activation functions are designed for $\Theta(1)$ arguments.
\greg{D1 imposes something weaker than required for this consideration. Nevertheless, the end result is that the condition on norm automatically implies a condition on the entry sizes, because of TP.}
Recall that the norm of a $d$-element vector with $\Theta(1)$ entries is $\Theta(\sqrt{d})$.%
\footnote{We could in principle relax D1 for homogeneous nonlinearities, but we do not gain anything by doing so.}
D2 simply enforces that the network output be bounded.
% \footnote{
% We permit the network outputs to be \textit{smaller} than order one at initialization.
% Surprisingly, we will find in Section [SECTION] that proper feature learning at large width \textit{requires} vanishing network output at init.
% }
\textbf{D3 is our requirement of feature learning.}
Feature learning requires the hidden representations of a network to change nontrivially during training.
These changes must be of the same order as the original representations: if they are smaller, feature learning vanishes at large width, and if they are bigger, then the dynamics explode.
D4 enforces that learning at any layer changes the network output at the correct scale.

Our approach will be as follows.
In Section \ref{sec:heuristic_picture}, we will paint a simple picture of an MLP trained with our spectral scaling condition which retains proper feature learning at large width.
Then, in Section \ref{sec:derivation}, we will show that this picture is the \textit{only} one --- no other scaling satisfies desiderata D1-D4 --- and that our scaling is in fact equivalent to muP.


==> old_sections/experiment.tex <==
\section{An illustrative experiment}
\label{sec:exp}

In light of our spectral analysis, assessing whether a network is learning features is as simple as measuring key spectral quantities over training and confirming that they scale as expected.
Here we do precisely this in a toy experiment in which two ReLU MLPs using muP and NTP scalings respectively are trained on the same task.
We will clearly see the presence of feature learning in muP (and the lack thereof in the NTP) reflected in spectral measurements.%
\footnote{A notebook reproducing this experiment is available at \texttt{[Colab url redacted for review]}.}

\newcommand{\toyexpntrain}{512}
\newcommand{\toyexpntest}{512}
\newcommand{\toyexpwidth}{4000}
We train three-hidden-layer FCNs on \toyexpntrain\ training samples from a two-class subset of CIFAR-10.
The initialization scales and layerwise learning rates for each are obtained by starting from the same width-1 base network and scaling up to width \toyexpwidth\ according to the parameterization's scaling prescription.
Each is trained with the same global learning rate, and each sees a $\Theta(1)$ decrease in the loss.
The results, shown in Figure \ref{fig:toy_fcn_exp}, strikingly illustrate that the muP net's hidden vectors, weight matrices, and last-layer alignment undergo leading-order updates relative to their values at initialization, while these changes are very suppressed for the NTP.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/relu_fcn_spectral_exp.pdf}
    \caption[]{
    \textbf{A wide ReLU FCN sees significant feature learning and weight matrix updates using muP scalings but not with NTP scalings.}
    \textit{Left:} Loss trajectories for two ReLU FCNs trained on a two-class subset of CIFAR-10.
    \textit{Center:} Relative updates to preactivation vectors, averaged over train samples\footnotemark.
    \textit{Right:} Relative spectral norm updates to weight matrices.
    \jamie{TODO: update figure and add traces of last-layer alignment. Note to self: think about how to modify the experiment to give higher last-layer alignment if needed.}
    }
    \label{fig:toy_fcn_exp}
\end{figure}

% This feature learning is also reflected in $\mathbb{E}_\vx \mathcal{A}(\mW_3, \vz_2)$,  the training-set average alignment between the last layer and its incoming activations, which is $\sim .16$ for the muP network and $\sim .008$ for the NTP network.\todo{Does this makes sense / seem worth including? Could also make it part of the figure}

==> old_sections/extensions.tex <==
\section{Extensions: additional steps, nonlinearities, and larger batch size}
\label{sec:extensions}

We now extend our warmup example to successively more general settings.
The point of each of these is that our spectral scaling condition remains sufficient to achieve feature evolution of the proper size.
The main intuitions from our warmup will carry through as we add complexity.

\subsection{Additional gradient steps}

Our warmup argument relied on two properties of $\mW_\ell$ at initialization: its spectral norm being the correct size (Condition \ref{cond:scaling}) and its passing forward a $\vh_\ell(\vx)$ of the correct size (Claim \ref{claim:update}).
Fortunately, it is easily seen that these properties are unchanged by the gradient step and we can therefore treat the second (and later) steps exactly as we did the first.

\textbf{Spectral norm remains the correct size.}
By the triangle inequality, we see that
\begin{equation}
    \norm{\mW_\ell + \DW_\ell}_*
    = \Theta \left( \norm{\mW_\ell}_* + \norm{\DW_\ell}_* \right)
    % = \sqrt{\frac{d_\ell}{d_{\ell-1}}}.
    = \Theta( \sqrt{d_\ell / d_{\ell-1}} )
\end{equation}
so long as $\mW_\ell$ and $\DW_\ell$ do not perfectly cancel, which is unlikely.

\textbf{The subsequent hidden vector remains the correct size.}
Recall that this property served to ensure (and was equivalent to) the desideratum that $\norm{\vh_\ell(\vx)}_2 = \Theta(\sqrt{d_\ell})$ --- that is, that the subsequent hidden vector was the correct size.
Fortunately, we can easily verify that the the updated hidden vector is still the same size: we again see by the triangle inequality that
\begin{equation}
    \norm{\vh_\ell(\vx) + \Delta \vh_\ell(\vx)}_2
    =
    \Theta(\norm{\vh_\ell(\vx)}_2 + \norm{\Delta \vh_\ell(\vx)}_2)
    =
    \Theta(\sqrt{d_\ell}),
\end{equation}
again assuming that $\vh_\ell(\vx)$ and $\Delta \vh_\ell(\vx)$ do not perfectly cancel, which is unlikely.
The intuition with both these observations is that the norms of weight matrices and hidden vectors only change by $\Theta(1)$ factors during training (as one expects from a stable dynamical process).

With these facts in place, the same argument we used in Section [SECTION] for the first step ensures that Desideratum \ref{des:scaling} also holds at the second and later steps.

% \begin{equation}
%     \norm{(\mW_\ell + \DW_\ell) \vh_{\ell-1}(\vx)}_2
%     =
%     \Theta
%     \left(
%     \norm{\vh_\ell(\vx)}_2 + \norm{\Delta \vh_\ell(\vx)}_2
%     \right)
%     % \Theta
%     % \left(
%     % \norm{\mW_\ell \vh_{\ell-1}(\vx)}_2
%     % +
%     % \norm{\DW_\ell \vh_{\ell-1}(\vx)}_2
%     % \right)
% \end{equation}

% We first extend our analysis of the first gradient step to subsequent steps on the same input using a recursive argument.
% Let us temporarily introduce the superscripts $\mW_\ell^{(t)}$, $\vh_\ell^{(t)}(\vx)$ to denote quantities after $t = \Theta(1)$ steps of gradient descent and denote the updates upon step $t$ by
% \begin{align}
%     \label{eqn:mWt_update_eqn}
%     \mW_\ell^{(t)} &= \mW_\ell^{(t-1)} + \DW_\ell^{(t)}, \\
%     \vh_\ell^{(t)}(\vx) &= \vh_\ell^{(t-1)}(\vx) + \Delta\vh_\ell^{(t)}(\vx).
% \end{align}

% Note that the only properties we required of $\mW_\ell^{(0)}$ in our warmup argument were (a) its norm obeying Condition \ref{cond:scaling} and (b) its alignment with incoming vectors.
% Fortunately, these properties are \textit{self-propagating} and thus hold at all $t$ in the following sense:
% \begin{claim}[Correct norm and alignment of $\mW_\ell^{(t)}$]
% \label{claim:Wkt_properties}
% Assume $\mW_\ell^{(t-1)}$ and $\DW_\ell^{(t)}$ obey Condition \ref{cond:scaling}.
% Then $\mW_\ell^{(t)}$ obeys
% \begin{equation*}
%     \norm{ \mW_\ell^{(t)} }_* = \Theta \left( \smash{\sqrt{d_\ell / d_{\ell-1}}} \right)
%     \qquad
%     \text{and}
%     \qquad
%     \norm{ \mW_{\ell}^{(t)} \vh_{\ell-1}^{(t)}(\vx)}_2 = \Theta \left( \norm{\mW_{\ell}^{(t)}}_* \cdot \norm{\vh_{\ell-1}^{(t)}(\vx)}_2 \right).
% \end{equation*}
% \end{claim}
% To verify the first part of this claim, note that so long as the first two terms in Equation \ref{eqn:mWt_update_eqn} do not perfectly cancel, it will hold that $\norm{\mW_\ell^{(t)}}_* = \Theta \left( \norm{\mW_\ell^{(t-1)}}_* + \norm{\DW_\ell^{(t)}}_* \right)$, and the r.h.s. is $\Theta \left( \smash{\sqrt{d_\ell / d_{\ell-1}}} \right)$ by assumption.
% The second part of the claim follows from the fact that $\DW_\ell^{(t)}$ aligns with $\vh_\ell^{(t-1)}(\vx)$ (and also assumes an unlikely perfect cancellation does not occur) and can be easily verified starting from the fact that
% \begin{equation}
%     \mW_{\ell}^{(t)} \vh_{\ell-1}^{(t)}(\vx) =
%     \left(
%     \mW_{\ell}^{(t-1)} + \DW_{\ell}^{(t)}
%     \right)
%     \left(
%     \vh_{\ell-1}^{(t-1)}(\vx) + \Delta\vh_{\ell-1}^{(t)}(\vx)
%     \right).
% \end{equation}
% The intuition to take away here is that each weight matrix will be aligned with incoming vectors after one or more gradient updates (which are themselves aligned with incoming vectors).

% Claim \ref{claim:Wkt_properties} assures us that $\mW_\ell^{(t)}$ obeys the properties we asked of $\mW_\ell^{(0)}$ in our warmup argument.
% We can thus reuse our argument recursively in $t$ to conclude that, so long as we continue to scale $\DW_\ell^{(t)}$ according to Condition \ref{cond:scaling}, we will obey Desideratum \ref{des:scaling} and achieve proper feature evolution at all $t$.

\subsection{Nonlinearities}

We now add a nonlinearity $\phi$ to each layer of our MLP.
The modified forward recursion relation is
\begin{equation}
    \vh_\ell(\vx) = \mW_\ell \vh'_{\ell-1}(\vx),
    \qquad
    \vh'_\ell(\vx) = \phi(\vh_\ell(\vx));
    \qquad
    \text{for } \ell = 2 \ldots L\!-\!1,
\end{equation}
with base case $\vh_1(\vx) = \mW_1 \vx$ and output $\vh_L(\vx) = \mW_L \vh'_{L-1}(\vx)$.
It will generally be the case that
\begin{equation}
    \norm{\vh'_\ell(\vx)}_2 = \Theta\left(\norm{\vh_\ell(\vx)}_2\right),
\end{equation}
and thus we may apply Desideratum \ref{des:scaling} equally well to either $\vh_\ell$ or $\vh'_\ell$.
As in the linear case, $\DW_\ell$ will be rank-one and align to incoming signal as
\begin{equation}
    \norm{\DW_\ell \vh'_\ell(\vx)}_2 = \norm{\DW_\ell}_* \cdot \norm{\vh'_\ell(\vx)}_2
\end{equation}
at each step.
All our scaling arguments from the linear case therefore carry through, and Condition \ref{cond:scaling} still achieves proper feature evolution.

\subsection{Batch size greater than one}

Observe that, when training on a minibatch $\mathcal{D} = \{(\vx_i, \vy_i)\}_{i=1}^n$ with size $n > 1$, each gradient step is simply an average of the steps on each example as
\begin{equation} \label{eqn:DWk_sum}
    \DW_\ell = \frac{1}{n} \sum_{i=1}^n \DW_\ell^{(i)}
\end{equation}
where the sum runs over the minibatch index and $\DW_\ell^{(i)}$ denotes the update that would result from a step on the single example $(\vx_i, \vy_i)$.
While $\DW_\ell$ is generally no longer rank one and cannot perfectly align to all $n$ incoming vectors, application of Equation \ref{eqn:DWk_sum} reveals that at least one summand will align to every $\vh_\ell(\vx_i)$.
We thus have that
\begin{equation} \label{eqn:batch_update_alignment}
    \norm{\DW_\ell \vh_\ell(\vx_i)}_2 =
    \Theta \left(
    \frac{1}{n}
    \norm{\DW_\ell}_*
    \norm{\vh_\ell(\vx_i)}_2
    \right)
    = \Theta \left(
    \norm{\DW_\ell}_*
    \norm{\vh_\ell(\vx_i)}_2
    \right).
\end{equation}
for all $i$, where in the second equality we have used the fact that $n = \Theta(1)$ by assumption (i.e. it remains fixed even when width is large).
Our previous scaling arguments in fact needed only alignment in the ``big-$\Theta$'' sense of Equation \ref{eqn:batch_update_alignment} (as opposed to the perfect rank-one sense of Claim \ref{claim:update}), and thus they still carry through: our spectral scaling condition continues to suffice to achieve proper feature learning as per Desideratum \ref{des:scaling}.


==> old_sections/heuristic_picture.tex <==
\section{A spectral picture of feature learning}
\label{sec:heuristic_picture}

Here we give a heuristic picture showing that our spectral scaling condition (Equation [EQUATION]) is enough to see proper feature learning in wide MLPs, and that furthermore this success is easily understood via the telescoping property.
It will turn out that the first gradient step requires special treatment (as it will tend to align initially-random tensors), and so it will prove simpler to first examine a network in the middle of training for which this has already happened.
We will return to initialization in Section \ref{sec:derivation}.

For simplicity, we will study a deep MLP with no biases and examine the effect of a single gradient step.
Because we are solely concerned with scaling with respect to hidden layer widths, our conclusions will be insensitive to the size of the data minibatch (so long as it remains constant), and so we will consider training on only a \textit{single input vector} $\vx$.
Similarly, it will turn out that including nonlinear activation functions does not affect our scaling analysis, so we drop them and study a deep \textit{linear} MLP.%
\footnote{To gain intuition for why activation functions do not affect scaling analysis, note that an activation function maps $\Theta(1)$ arguments to $\Theta(1)$ outputs and thus does not change the magnitude of a hidden vector as far as scaling with width is concerned.}
We refer interested readers to Appendix [APPENDIX] for a version of this section with nonlinearities included.

\subsection{The model: a deep linear MLP}
Consider a depth-$L$ MLP with layer widths $\{d_\ell\}_{\ell = 0}^L$.
All $d_\ell$ will grow large (possibly at different rates) except $d_0$ and $d_L$, which will remain constant.
Let the network have weight matrices $\{ \mW_\ell \}_{\ell=1}^L$ with $\mW_\ell \in \R^{d_{\ell-1} \times d_\ell}$.
We consider a single input $\vx$ with $\Theta(1)$ entries and thus norm $\norm{\vx}_2 = \Theta(d_0)$.
The forward propagation of the network is given by
\begin{equation} \label{eqn:linear_mlp_forwardprop}
    \vh_1(\vx) = \mW_1 \vx,
    \qquad
    \vh_\ell(\vx) = \mW_\ell \vh_{\ell-1}(\vx)
    \ \ \ \ \
    \text{for $\ell = 2 \ldots L$},
\end{equation}
with $\vh_L(\vx)$ the output of the network.
Because we have only one input, we will henceforth simply write $\vh_\ell$ for the hidden vector at layer $\ell$.

We will write $\Delta \mW_\ell$ for a gradient update to $\mW_\ell$ and $\Delta \vh_\ell$ for the resulting update to $\vh_\ell$.
To disentangle the effects of training at different layers, we will generally consider performing a gradient update at just one layer at a time.
Which layer is updated will be clear from context.

Condensing D1-D4, we desire the following:
\begin{equation} \label{eqn:feature_learning_condn}
    \norm{\vh_\ell}_2 \sim \norm{\Delta \vh_\ell}_2 = \Theta(\sqrt{d_\ell})
    \ \ \ \ \
    \text{for}
    \ \ \ \ \
    \ell = 1 \ldots L.
\end{equation}

\subsection{First look: upper bounds on feature norms}

It is easy to see that we will not \textit{exceed} the scaling mandated by Equation \ref{eqn:feature_learning_condn} so long as $\norm{\mW_\ell}_* \sim \norm{\Delta \mW_\ell}_* = \Theta \left(\sqrt{\frac{d_\ell}{d_{\ell-1}}} \right)$:
Before the gradient step, each feature vector obeys the upper bound
\begin{equation} \label{eqn:ub_1}
    \norm{\vh_\ell}_2
    = \norm{\mW_\ell \cdots \mW_1 \vx}_2
    {\color{red}{\le}} \norm{\mW_\ell}_* \cdots \norm{\mW_1}_* \norm{\vx}_2
    = \Theta \left( \sqrt{\frac{d_\ell}{d_{\ell-1}}} \cdots \sqrt{\frac{d_1}{d_0}} \sqrt{d_0} \right)
    % = \prod_{\ell'=1}^\ell \Theta(\sqrt{\frac{d_\ell}{d_{\ell-1}}})
    = \Theta(\sqrt{d_\ell})
\end{equation}
and thus $\norm{\vh_\ell}_2 = \O(\sqrt{d_\ell})$.
After an update at layer $\ell$, the change at layer $\ell \ge \ell$ is bounded by
\begin{multline} \label{eqn:ub_2}
    \norm{\Delta \vh_\ell}_2
    = \norm{\mW_\ell \cdots \mW_{\ell+1} \Delta \mW_\ell \vh_{\ell-1}}_2
    {\color{red}{\le}} \norm{\mW_\ell}_* \cdots \norm{\mW_{\ell + 1}}_* \norm{\Delta \mW_\ell}_* \norm{\vh_{\ell-1}}_2 \\
    = \Theta \left( \sqrt{\frac{d_\ell}{d_{\ell-1}}} \cdots \sqrt{\frac{d_\ell}{d_{\ell-1}}} \sqrt{d_{\ell-1}} \right)
    = \Theta(\sqrt{d_\ell})
\end{multline}
and thus $\norm{\Delta \vh_\ell}_2 = \O(\sqrt{d_\ell})$.

\subsection{The aligning effect of gradient descent}

To show that these bounds are tight, we must consider the aligning effect of gradient descent.
Let us suppose we train to minimize a loss $\L = \L(\vh_L, \vy)$ where $\vy$ is a target vector.
We will update each layer via gradient descent as
$\Delta \mW_\ell = - \eta_\ell \nabla_{\mW_\ell} \L$,
where $\eta_\ell$ is a layerwise learning rate to be determined.
The parameter gradients are given via the rank-one outer product
\begin{equation}
    \nabla_{\mW_\ell} \L = \vg_\ell \vh_{\ell-1}\T,
\end{equation}
where $\vg_\ell \defeq \nabla_{\vh_\ell} \L$ is the gradient vector at layer $\ell$ given via backpropagation as
\begin{equation} \label{eqn:linear_mlp_backprop}
    \vg_L = \nabla_{\vh_L} \L,
    \qquad
    \vg_\ell = \mW_\ell\T \vg_{\ell+1}
    \ \ \ \ \
    \text{for}
    \ \ \ \ \
    \ell = (L-1) \ldots 1.
\end{equation}
From the fact that $\Delta \mW_\ell \propto \vg_\ell \vh_{\ell-1}\T$,
we can make an important observation: \textit{gradient updates to weight tensors act maximally}.
This is true both for the forward propagation of signal and the backward propagation of gradients:
\begin{equation}
    \alignment(\Delta \mW_\ell, \vh_{\ell-1}) = \alignment(\Delta \mW_\ell\T, \vg_\ell) = 1.
\end{equation}

Because updates to weight matrices act maximally, it is reasonable to assume that after several gradient steps all tensors are aligned and the network is fully maximal:

\begin{assumption}[Fully maximal network] \label{assumption:full_maximality}
% $\alignment(\Delta \mW_\ell, \vh_{\ell-1}) \sim \alignment(\Delta \mW_\ell\T, \vg_\ell) = \Theta(1)$ for all $\ell = 1 \ldots L$.
Every weight matrix $\mW_\ell$ acts maximally on both forward signal $\vh_{\ell-1}$ and backwards gradient $\vg_\ell$.
\end{assumption}

With Assumption \ref{assumption:full_maximality}, the telescoping property permits us to replace ``${\color{red}{\leq}}$" with ``${\color{red}{\sim}}$" in both Equations \ref{eqn:ub_1} and \ref{eqn:ub_2}.%
\footnote{To see why this is true of Equation \ref{eqn:ub_2}, note that $\vg_\ell = (\mW_\ell \cdots \mW_{l+1})\T \vg_\ell$ and thus Proposition \ref{prop:align_properties}(d) implies that $\alignment(\mW_\ell \cdots \mW_{l+1}, \vg_\ell) = \Theta(1)$ given Assumption \ref{assumption:full_maximality}.}
We therefore have properly-scaled network dynamics:

\begin{tcolorbox}[colback=white, colframe=black, boxrule=1pt, arc=0pt]
\begin{proposition}[Spectral scalings give feature learning]
Given Assumption \ref{assumption:full_maximality}, weight scalings obeying Condition \ref{cond:scaling} yield
\begin{equation}
    \norm{\vh_\ell}_2 \sim \norm{\Delta \vh_\ell}_2 = \Theta(\sqrt{d_\ell}).
\end{equation}
\end{proposition}
\end{tcolorbox}
\jamie{Thoughts on making this a proposition? Last-minute change on my part. Draws attention to it, but is perhaps unnecessary.}

We also have the following nice corollary:
\begin{corollary}[Update-gradient alignment] \label{cor:update-grad-align}
Given Assumption \ref{assumption:full_maximality}, weight scalings obeying Condition \ref{cond:scaling}
\begin{equation}
    \alignment(\vg_\ell, \Delta \vh_\ell) = \Theta(1).
\end{equation}
\end{corollary}
That is, features update in a direction with $\Theta(1)$ alignment with the direction they ``wanted to go" even when the gradient step occurs at an earlier layer.
We give the proof in Appendix [APPENDIX].




% We will argue that, for proper feature learning, a network should be \textit{fully maximal upon both forward- and backprop} in the sense that every matrix-vector multiply in Equations \ref{eqn:linear_mlp_forwardprop} and \ref{eqn:linear_mlp_backprop} has $\Theta(1)$ alignment.
% Heuristically speaking, both the forward and backward signals have to ``see" the true size of each matrix.\footnote{This is a very reasonable condition: recall from Section \ref{sec:preliminaries} that it is already true for most weight matrices at init.}
% We will shortly show that this full maximality is in fact a requirement, and that scalings which fail to learn features fail because they do not arrive at a fully-maximal state.
% For now, however, \textit{we simply assume that our MLP is fully maximal}.

% \subsection{[SUBSECTION NAME]}

% Our learning desiderata D3 and D4 can be summarized as follows:
% \begin{itemize}
%     \item Updating $\mW_\ell$ via a gradient step causes a change $\norm{\Delta \vh_\ell}_2 = \Theta(\sqrt{d_\ell})$ for $\ell = \ell \ldots L$.
% \end{itemize}
% Recall that the norm of a $d$-vector with $\Theta(1)$ entries is $\Theta(\sqrt{d})$.

% - posit the spectral conversion condition
% - show that it's right upon forward prop
% - give the scalings of the g's upon backprop
% - show that it satisfies our FL condition upon a gradient step



% assume full maximality.
% show that the spectral scaling condition satisfies the desiderata.
% show that without full maximality, we cannot satisfy both D3 and D4 with any scaling.
% (but you don't need full maximality at init... what's going on?)
% (ah, I see... it's not really about full maximality, it's about the requirement that every tensor acts with the same norm forwards and backwards. except for the last layer, which it's fine if it acts with a small norm forwards. and the first layer, for which it doesn't matter how it acts backwards.)


==> old_sections/nondimensionalization.tex <==
\section{Nondimensionalizing neural network dynamics}
\label{sec:nondimensionalization}

We have shown that, for proper feature learning, each layer of a network must satisfy a spectral condition (Condition \ref{cond:scaling}) which depends on the dimensionalities of the neighboring layers.
In this brief section, we show that this condition can be \textit{nondimensionalized}, reducing to the satisfying requirement that ``all interesting quantities are order one."
This is akin to similar simplifications used widely across fields of physics.
This section is written for ``advanced users" of our spectral view, and we suggest reading Sections \ref{sec:intro}-\ref{sec:derivation} first.

We begin by defining a rescaled version of the $\ell^2$-norm:
\begin{definition}[Rescaled $\ell^2$-norm]
The rescaled $\ell^2$-norm of a vector $\vv \in \R^m$ is
\begin{equation}
    \nnorm{\vv}_2 \defeq \frac{1}{\sqrt{m}} \norm{\vv}_2.
\end{equation}
\end{definition}
This norm returns the typical entry size of a vector (specifically the root-mean-square entry size) regardless of its dimensionality.
We also define a modified spectral norm:
\begin{definition}[rescaled spectral norm]
The rescaled spectral norm of a matrix $\mA \in \R^{m \times n}$ is
\begin{equation}
    \nnorm{\mA}_* \defeq \frac{\sqrt{m}}{\sqrt{n}} \norm{\mA}_*.
\end{equation}
\end{definition}
The standard spectral norm is the norm induced by the standard $\ell^2$-norm, and this is also true of their rescaled variants.

Using these rescaled norms, we find that our scaling condition has become nondimensionalized:
\begin{tcolorbox}[colback=white, colframe=black, boxrule=1pt, arc=0pt]
  \begin{condition}[Spectral scaling, nondimensionalized] \label{cond:scaling_nondim}
    The weight matrices of a neural network and their gradient updates should satisfy
    \begin{align*}
        \nnorm{\mW_\ell}_* \sim \nnorm{\Delta \mW_\ell}_* \sim 1
        \qquad \text{ at all layers } \ell=1,...,L.
    \end{align*}
\end{condition}
\end{tcolorbox}

For good measure, we also give nondimensionalized versions of desiderata D1-D4:
\begin{enumerate}[leftmargin=1.2cm,itemsep=0pt,topsep=0pt,label=\textbf{\textlangle D\arabic*'\textrangle}]
\item
At initialization, $\nnorm{\vh_\ell(\vx)}_2 = \Theta(1)$ for $\ell = 1 \ldots L-1$.
% During training, the network output $\vh_L(\vx)$ must be $\mathcal{O}(1)$.
\item At initialization, $\nnorm{\vh_L(\vx)}_2 = \O(1)$.
\item
Performing a gradient step at layer $\ell$ must induce updates $\nnorm{\Delta \vh_\ell(\vx)} = \Theta(1)$ for $\ell = \ell \ldots L-1$ at all subsequent hidden layers.
\item
% Performing a gradient step at any layer must effect $\Theta(1)$ updates to the network output.
Performing a gradient step at layer $\ell$ must induce an update $\nnorm{\Delta \vh_L(\vx)} = \Theta(1)$ at the output.
\end{enumerate}
We note that the $\alignment(\cdot, \cdot)$ metric is the same whether the original or rescaled norms are used, and that all interesting matrix-vector alignments are also order one in a network learning features.
With this lens, checking network for proper feature learning is in principle as simple as computing interesting quantities at a few widths and confirming that they are all $\Theta(1)$ with respect to width.

==> old_sections/optimizers.tex <==
\section{Spectrally scaled optimizers}
\label{sec:optimizers}

\jamie{Jeremy to write! Discussion of spectral optimizer rules, contrast with Frobenius-normed rules, and experiments with deep nets.}

==> old_sections/path_heuristic.tex <==
\section{The heuristic of maximal paths}
\label{sec:path_heuristic}

Here we introduce a visual heuristic for reasoning about layerwise contributions to feature learning in deep neural networks.
At each layer $\ell$ of a deep network, let $\mW_\ell^0$ denote the weight tensor at initialization, let $\mW_\ell$ denote the weight tensor after a training procedure, and let $\Delta \mW_\ell = \mW_\ell - \mW_\ell^0$ denote the cumulative sum of all updates during training.
In a slight modification of prior notation, we denote the output of the network by $f(\vx) = f(\vx; \{\mW_\ell\}_\ell)$.

Heuristically speaking, we may conceive of the network output $f(\vx; \{\mW_\ell\}_\ell)$ as the totality of $2^L$ contributions in the following exact sense.
For a set of indices $\B \in [L]$, we define
\begin{equation}
    \tilde{f}_B(\vx) \defeq f \! \left( \vx; \{\mW_\ell^0 + \mathbbm{1}_{\ell \in \B} \cdot \Delta \! \mW_\ell\}_\ell \right).
\end{equation}
That is, $\tilde{f}_B(\vx)$ is the network output if only layers $\ell \in \B$ are updated from their initial states.

We wish to isolate the joint contribution to the output due to the updates at a subset of layers.
To that end, we define the joint contribution
\begin{equation} \label{eqn:incl_excl}
    f_\B(\vx) \defeq \sum\limits_{\B' \subseteq \B} (-1)^{|\B - \B'|} \tilde{f}_{\B'}(\vx).
\end{equation}
This isolates the joint contribution of the updates at layers in $\B$ via the inclusion-exclusion principle.%
\footnote{To build intuition for Equation \ref{eqn:incl_excl}, it is useful to write out a few lower-order terms explicitly. For example, $f_\emptyset(\vx) = \tilde{f}_\emptyset(\vx)$ is the function at initialization, and $f_{\{\ell\}}(\vx) = \tilde{f}_{\{\ell\}}(\vx) - \tilde{f}_\emptyset(\vx)$ is the change due to updating layer $\ell$.}
Note that these contributions sum up to the total function:
\begin{equation}
    f(\vx) = \sum_\B f_\B(\vx).
\end{equation}
We may interpret $f_\B(\vx)$ as either the joint contribution of a subset of updates or as the contribution of a particular ``path" through the network: that is, a path from input to output which passes through either $\mW_\ell^0$ or $\Delta \mW_\ell$ at each layer depending on whether $\ell \in \B$, with the full output being the sum of the contributions of all $2^L$ paths.

It is illuminating to examine the relative contributions of subsets $\B$ of different cardinality for networks that do and do not learn features.
A simple scaling analysis like those of Sections \ref{sec:heuristic_picture} and \ref{sec:derivation} easily shows that, for a network trained using the NTP, we have:
\begin{equation} \label{eqn:contrib_orders_ntp}
    f^{\text{(NTP)}}_\B(\vx) =
    \begin{cases}
        \Theta(1) & \text{if } |\B| = 0 \\
        \Theta(1) & \text{if } |\B| = 1 \\
        o(1) & \text{if } |\B| > 1.
    \end{cases}
\end{equation}

That is, when using the NTP, \textit{only linear perturbations in the weights affect the output to leading order}.
This is reflects the linearity of training in the the lazy (i.e. ``kernel") regime.
This absence of interactions signifies a lack of feature learning: each layer has updated independently, and this is because changes propagated from updates at early layers are too small to be seen by later layers.%
\footnote{This illustrates the ``dynamical dichotomy theorem" of [CITATION]: with any parameterization, one may have either feature learning or linear dynamics, but not both.}
% Note that any network whose features evolve to leading order will also have leading-order interactions between updates at different layers: feature evolution is due to change at earlier layers, and later layers then couple to the changed features, leading to at least 2nd-order interactions at leading order.

The scalings for muP are as follows:
\begin{equation} \label{eqn:contrib_orders_mup}
    f^{\text{(muP)}}_\B(\vx) =
    \begin{cases}
        o(1) & \text{if } |\B| = 0 \\
        \Theta(1) & \text{if } |\B| = 1 \\
        \Theta(1) & \text{if } |\B| > 1.
    \end{cases}
\end{equation}
That is, in muP, \textit{update interactions of all degrees matter to leading order}.
These higher-order interactions are an inevitable in a network learning features: feature evolution is due to change at earlier layers, and later layers then couple to the changed features, leading to at least 2nd-order interactions at leading order.

\jamie{I totally just quoted the above facts without proof. They're not really hard to show (I think) but are sort of annoying to write out, esp with nonlinearities. If there's a nice way to just say ``this is true and we leave showing it as an exercise to the reader," I'd like to do that.}

In addition to asking whether a particular path contributes to the output at leading order, we may also ask whether a path is \textit{maximal} in the following sense.
The path corresponding to a subset $\B$ passes through the set of parameters
\begin{equation}
    \mathcal{W}^{(\B)} = \{\mathbbm{1}_{\ell \notin \B} \cdot \mW_\ell^0 + \mathbbm{1}_{\ell \in \B} \cdot \Delta \! \mW_\ell\}_\ell.
\end{equation}
We will say a path is maximal if
\begin{equation}
    |f_\B(\vx)|
    = \Theta \left(
    \prod_\ell \norm{\mathcal{W}^{(\B)}_\ell}_*
    \cdot
    \norm{\vx}_2
    \right).
\end{equation}
That is, a path is maximal if its contribution to the output is of the largest order possible given the spectral norms of its components.

The path maximalities of the NTP and muP are given by the following table:
\begin{center}
\begin{tabular}{cccc}
& $|\B|=0$ & $|\B|=1$ & $|\B|>1$ \\ \hline \rule{0pt}{4mm}
NTP maximal? & \xmark & \cmark & \xmark \\
muP maximal? & \xmark & \cmark & \cmark
\end{tabular}
\end{center}

While only degree-one paths are maximal for the NTP, all paths except the degree-zero path are maximal in muP.
Note that because the degree-zero path is never maximal due to dimensionality considerations (Section \ref{sec:derivation}), this means that muP is ``as maximal as possible," hence the name ``maximal update parameterization."

\subsection{Special case: deep linear network}

In the case in which the network has no pointwise nonlinearities, we have
\begin{equation} \label{eqn:deep_linear_product}
    f(\vx)
    =
    ( \mW_L^0 + \Delta \mW_L) \cdots ( \mW_1^0 + \Delta \mW_1) \vx.
\end{equation}
Note that we may expand the right hand side of Equation \ref{eqn:deep_linear_product} into the sum of $2^L$ terms, each of which is precisely $f(\vx; \mathcal{W}^{(\B)})$ for a particular $\B$.
These are precisely the $2^L$ paths through the network: in the linear case, the function can be written explicitly as $2^L$ tensor contractions, one for each path.
The inclusion-exclusion sum of Equation \ref{eqn:incl_excl} simplifies greatly, and we find that
\begin{equation}
    f_\B (\vx) = f \left( \vx; \mathcal{W}^{(\B)} \right).
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/path_heuristic_fig.png}
    \caption{
    \textbf{Pathwise decomposition of a deep linear network.}
    \textit{Left column:} depiction of combinatorial paths through a deep linear network with each weight matrix decomposed into initialization and total update as $\mW_\ell = \mW_\ell^0 + \Delta \mW_\ell$.
    Paths are grouped by the number of updates they include.
    \textit{Middle column:} Classification of paths under muP scalings in terms of (1) whether they contribute to $f(\vx)$ at leading order and (2) whether all weight matrices act maximally.
    The fact that paths with many interactions are still leading-order is indicative of feature learning.
    \textit{Right column:} Similar classification of paths for the NTP.
    [TODO: add extra two paths in bottom left box; explicitly state the term associated with one of the paths; clarify that the rows aren't number of steps, they're number of interactions]
    }
    \label{fig:paths}
\end{figure}

\subsection{Visualizing paths}

Figure \ref{fig:paths} gives a visual depiction of the $2^L$ paths through a linear network with $L=3$.
We separate paths with $|\B| = 0$, $|\B| = 1$, and $|\B| > 1$ and note whether each path is (a) leading-order and (b) maximal when training with the NTP and with muP.
Paths of high update degree are leading-order and maximal in muP, which is indicative of feature learning.

These diagrams are cousins of Feynman diagrams in physics, which also depict possible dynamical paths whose contributions must be summed.
Prior work has used Feynman diagrams to study the NTP with perturbative corrections for large-but-finite width in an effort to describe feature learning [CITATIONS].
Our path heuristic suggests this approach may be bound to fail: high-order interactions (paths with many $\Delta \mW_\ell$'s) contribute to \textit{leading order} in proper feature learning, and are thus \textit{not perturbative}.
Specifically, any attempt to perturb to finite update degree will miss leading-order effects.%
\footnote{While our discussion here may make it seem like a perturbation up to order $L$ may be sufficient, in practice these perturbative approaches must deal with interactions not only across all layers but also between updates made at all steps of gradient descent, which quickly becomes too much to keep track of.
See [CITATION] for a dynamical mean field theory approach to tracking these correlations without relying on finite-width perturbation theory.}
This implies that, in the typical language of physics, a neural network learning features is a \textit{strongly-interacting system}.

% \footnote{Note that the sole relevance of first-order terms in the NTP scaling also signifies that the training dynamics are linear. This illustrates the dynamical dichotomy theorem of [CITATION]: with any parameterization, one may have either feature learning or linear dynamics, but not both.}%
% \footnote{Our diagrams are cousins of Feynman diagrams in physics, which also depict possible dynamical paths whose contributions must be summed. Prior work has used Feynman diagrams to study the NTP with perturbative corrections for large-but-finite width in an effort to describe feature learning [CITATIONS]. Our path heuristic suggests this approach may be bound to fail: high-order interactions (paths with many $\Delta \mW_\ell$'s) contribute to \textit{leading order} in proper feature learning, and are thus \textit{not perturbative}.}%



==> old_sections/proofs.tex <==
\section{Proofs}
\label{app:proofs}

\subsection{Alignment}

\begin{proposition}[Properties of alignment] \label{prop:align_properties}
For any compatible tensors $\mP, \mQ, \mR$, the following hold:
\begin{enumerate}[(a)]
    \item $\alignment(\mP, \mQ) \in [0,1]$ \hfill (values in unit interval) \label{property:unit}
    \item $\alignment(\mP, \mP\T) = 1$ \hfill (reflexivity) \label{property:refl}
    \item $\alignment(\mP, \mQ) \times \alignment(\mP \mQ, \mR) = \alignment(\mP, \mQ \mR) \times \alignment(\mQ, \mR)$ \hfill (associativity) \label{property:assoc}
    \item $\alignment(\mP\T, \mP \mQ) \ge \alignment(\mP, \mQ)$ \hfill (iterativity) \label{property:iter}
    % \item $\alignment(\mP \mQ, \mR) \ge \alignment(\mP, \mQ \mR) \times \alignment(\mQ, \mR)$ \hfill (chain bound)
\end{enumerate}
\end{proposition}

\begin{proof}

Here we provide proofs of the four properties of Proposition \ref{prop:align_properties}.
Recall that alignment is defined as
\begin{equation} \label{eqn:alignment_def}
    \alignment(\mP, \mQ) \defeq \frac{\norm{\mP \mQ}_*}{\norm{\mP}_* \norm{\mQ}_*}.
\end{equation}
% Recall also that the spectral norm of a matrix $\mP \in \R^{m \times n}$ is given by
% \begin{equation} \label{eqn:spectral_norm_max_form}
%     \norm{\mP}_* = \max_{\substack{\vu \in \R^n \\ \norm{\vu}_2 = 1}} \norm{\mP \vu}_2.
% \end{equation}
% This definition also applies to vector $\mP$, using $m=1$ (for row vectors) and $n=1$ (for column vectors).

\textbf{Property (a):} $\alignment(\mP, \mQ) \in [0,1]$.

Alignment is nonnegative because the spectral norm is nonnegative.
Alignment is less than one because the spectral norm is submultiplicative.

\textbf{Property (b):} $\alignment(\mP, \mP\T) = 1$.

Let $\sigma_* = \norm{\mP}_*$ be the top singular value of $\mP$.
It follows immediately from the singular value decomposition that $\norm{\mP \mP\T}_* = \sigma_*^2$.
We thus have that
\begin{equation}
    \alignment(\mP, \mP\T)
    = \frac{\norm{\mP \mP\T}_*}{\norm{\mP}_*^2}
    = \frac{\sigma_*^2}{\sigma_*^2} = 1,
\end{equation}
where we have used the fact that $\norm{\mP}_* = \norm{\mP\T}_*$.

\textbf{Property (c):} $\alignment(\mP, \mQ) \times \alignment(\mP \mQ, \mR) = \alignment(\mP, \mQ \mR) \times \alignment(\mQ, \mR)$.

Writing out both sides of the equality explicitly, we observe that
\begin{equation}
    \frac{\norm{\mP \mQ}_*}{\norm{\mP}_* \norm{\mQ}_*}
    \frac{\norm{\mP \mQ \mR}_*}{\norm{\mP \mQ}_* \norm{\mR}_*}
    =
    \frac{\norm{\mP \mQ \mR}_*}{\norm{\mP}_* \norm{\mQ}_* \norm{\mR}_*}
    =
    \frac{\norm{\mP \mQ \mR}_*}{\norm{\mP}_* \norm{\mQ \mR}_*}
    \frac{\norm{\mQ \mR}_*}{\norm{\mQ}_* \norm{\mR}_*}.
\end{equation}

\textbf{Property (d):} $\alignment(\mP\T, \mP \mQ) \ge \alignment(\mP, \mQ)$.

We wish to prove that
\begin{equation}
    \frac{\norm{\mP\T \mP \mQ}_*}{\norm{\mP\T}_* \norm{\mP \mQ}_*}
    \ge
    \frac{\norm{\mP \mQ}_*}{\norm{\mP}_* \norm{\mQ}_*}
    \ \ \ \ \
    \Leftrightarrow
    \ \ \ \ \
    \norm{\mQ}_* \norm{\mP\T \mP \mQ}_*
    \ge
    \norm{\mP \mQ}_*^2
    = \norm{\mQ\T \mP\T \mP \mQ}_*,
\end{equation}
where in the last step we have used property (b).
The right-hand inequality is true by the submultiplicativity of the spectral norm.
\end{proof}


==> old_sections/short-derivation-jamie.tex <==
\section{The spectral scaling condition induces feature learning}
\label{sec:warmup}

% what should the section title be? it's not that it's a toy derivation. it's not that it's a warmup -- it really captures the core intuition of the spectral scaling. it's sort of a simple example? it's not really a derivation -- we're not deriving anything.

Here we demonstrate the correctness of Condition \ref{cond:scaling} in a simple model: a deep linear MLP trained for one step on a single example.
While elementary, this example will be sufficient to capture the intuition for the fully general case, and we begin here for pedagogical clarity.

\textbf{Model definition.}
We will study an MLP composed of $L$ successive linear transformations.
We consider a single input $\vx \in \R^{d_0}$ with norm $\norm{\vx}_2 = \Theta(\sqrt{d_0})$.%
\footnote{This input scaling is standard for many common data formats including images.}
The first hidden representation is $\vh_1(\vx) = \mW_1 \vx$, with the rest of the network following recursively as
\begin{equation}
    \label{eqn:hk}
    \vh_{\ell}(\vx) = \mW_\ell \vh_{\ell-1}(\vx)
    \qquad
    \text{for } \ell = 2, \ldots L.
\end{equation}
We let $\vh_L(\vx) \in \R^{d_L}$ be the network output.
We will keep the input dimension $d_0$ and output dimension $d_L$ fixed and consider scaling with respect to the hidden dimensions $d_1, \ldots, d_{L \!-\! 1}$.

We let the global loss be $\L = \ell(\vh_L(\vx), \vy)$ where $\ell$ and $\vy$ are a loss function and target vector, respectively.
During training, we will take gradient steps at each layer as $\DW_\ell = - \eta_\ell \cdot \nabla_{\mW_\ell} \L$, where $\eta_\ell$ is a layerwise learning rate.
We will ultimately solve for the scale of $\eta_\ell$, but for now we will be content to discuss $\DW_\ell$ directly.
From Equation \ref{eqn:hk}, hidden vector updates at subsequent layers are related by
\begin{equation}
    \label{eqn:delta_hk}
    \vh_\ell(\vx) + \Delta \vh_\ell(\vx) = (\mW_\ell+\DW_\ell) (\vh_{\ell-1}(\vx) + \Delta \vh_{\ell-1}(\vx)).
\end{equation}

\textbf{Hidden vector sizes.}
To reiterate Desideratum \ref{des:scaling}, we wish for features at the $\ell$th layer to have norm which scales as $\norm{\vh_\ell}_2 = \Theta(\sqrt{d_\ell})$, for $\ell = 1\ldots L\!-\!1.$
Upon each gradient update, we wish this feature vector to undergo an update of size $\norm{\Delta \vh_\ell}_2 = \Theta(\sqrt{d_\ell})$.
We will show that Condition \ref{cond:scaling} is sufficient to achieve these aims.

\textbf{Plan of attack.}
For simplicity, we will first focus on the \textit{first step of gradient descent} after random initialization.
We will argue recursively in depth, showing that if the features at layer $\ell-1$ and their updates satisfy Desideratum \ref{des:scaling}, then so will those at layer $\ell$ if the weights and their updates are scaled according to Condition \ref{cond:scaling}.
In order to verify the desired scalings, we will show upper and lower scaling bounds separately: we will first show that the features and their updates are not ``too big,'' and then show that they are not ``too small.''

\textbf{Hidden vector updates.}
Applying the submultiplicativity of the spectral norm to Equations \ref{eqn:hk} and \ref{eqn:delta_hk}, we find that
\begin{align*}
    \norm{\vh_{\ell}(\vx)}_2 &\le \norm{\mW_\ell}_* \norm{\vh_{\ell-1}(\vx)}_2 = \Theta(\sqrt{d_\ell}); \\
    \norm{\Delta \vh_\ell(\vx)}_2 &\le
    \norm{\DW_\ell}_* \norm{\vh_{\ell-1}(\vx)}_2
    + \norm{\mW_\ell}_* \norm{\Delta \vh_{\ell-1}(\vx)}_2
    + \norm{\DW_\ell}_* \norm{\Delta \vh_{\ell-1}(\vx)}_2
    = \Theta(\sqrt{d_\ell}),
\end{align*}
where on the right hand sides of the inequality we have inserted Desideratum \ref{des:scaling} and Condition \ref{cond:scaling}.
We see our spectral scaling condition thus gives features and feature updates obeying the correct \textit{upper} bound.

\textbf{Tightness of bounds via matrix-vector alignment.}
We may now make the suggestive observation that the possible looseness in these bounds came from our ``approximating the norm of the product by the product of the norms" for various matrix-vector products.
We now argue that this is in fact a good approximation and conclude that these bounds are tight in a scaling sense.

The key observation is that both random hidden weight matrices and subsequent updates act maximally on incoming vectors.
We make these observations precise with the following claims:
\begin{claim}[Alignment of initial weight matrices]\label{claim:init}
Fix a feature vector $\vh_{\ell-1}(\vx)\in\R^{d_{\ell-1}}$.
Assume $\mW_\ell$ in $\R^{d_\ell\times d_{\ell-1}}$ is sampled using a common weight initialization strategy. Provided that $d_\ell = \Omega(d_{\ell-1})$, then with high probability:
    \begin{equation*}
        \norm{ \mW_{\ell}\vh_{\ell-1}(\vx)}_2 = \Theta (\norm{\mW_{\ell}}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2).
    \end{equation*}
\end{claim}
\begin{claim}[Alignment of updates]
\label{claim:update}
For an update $\DW_\ell$ given by gradient descent at batch size 1,
    \begin{equation*}
        \norm{ \Delta\mW_{\ell}\vh_{\ell-1}(\vx)}_2 = \norm{\DW_{\ell}}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2.
    \end{equation*}
\end{claim}
We now justify these claims in turn.
For Claim \ref{claim:init}, first observe that when $d_\ell = d_{\ell-1}$ and $\mW_\ell$ is a random \textit{orthogonal matrix}, we have \textit{equality} --- that is, $\norm{ \mW_{\ell}\vh_{\ell-1}(\vx)}_2 = \norm{\mW_{\ell}}_* \norm{\vh_{\ell-1}(\vx)}_2$.
When the elements of $\mW_\ell$ are instead sampled i.i.d. from a Gaussian or uniform distribution, standard results from random matrix theory show that a random matrix comes close to equality in this sense (so long as its aspect ratio is not too extreme), merely incurring a penalty of an order-one prefactor for not being orthogonal.
For example, so long as $d_\ell \ge d_{\ell-1}$, it holds that
\begin{equation}
    \norm{\mW_{\ell}\vh_{\ell-1}(\vx)}_2 \gtrsim \frac{1}{2} \norm{\mW_{\ell}}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2
    \qquad
    \text{with high probability.}
\end{equation}
For interested readers, we give a more detailed discussion and a review of relevant random matrix theory results in Appendix [APPENDIX].
The key takeaway is that \textit{all $\mW_\ell$ act on typical vectors with the same order as their spectral norm} so long as $d_\ell$ is not much less than $d_{\ell-1}$ (which, in a wide MLP with uniform hidden widths, only excludes the final layer $\mW_L$).

Claim \ref{claim:update} is easily verfied as follows.
Observe that we can directly write the update at layer $\ell$ as
\begin{equation} \label{eqn:DW}
    \DW_\ell = -\eta_\ell \cdot \nabla_{\vh_{\ell}(\vx)}\el \cdot \vh_{\ell-1}(\vx)^\top.
\end{equation}
Note that $\DW_\ell$ is rank-one and its one right singular vector is precisely $\vh_{\ell-1}(\vx)$, which verifies the claim.
Writing terms out explicitly for the purposes of pedagogy, we find that
\begin{equation}
    \norm{\DW_\ell \vh_{\ell-1}(\vx)}_2 = \eta_\ell \cdot
    \norm{\nabla_{\vh_{\ell}(\vx)}\el}_2
    \cdot \norm{\vh_{\ell-1}(\vx)}_2^2
    = \norm{\DW_\ell}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2.
\end{equation}

With these facts in place, we can now get lower bounds on hidden vector size which verify Desideratum \ref{des:scaling}.
The features at initialization scale correctly as
\begin{equation} \label{eqn:vh_l_tight_scaling}
    \norm{\vh_\ell(\vx)}_2
    = \Theta \left( \norm{\mW_\ell}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2 \right)
    % = \Theta \left( \sqrt{\frac{d_\ell}{d_{\ell-1}}} \cdot \sqrt{d_{\ell-1}} \right)
    = \Theta(\sqrt{d_\ell}),
\end{equation}
where we have first used Claim \ref{claim:init} and then inserted Condition \ref{cond:scaling}.
To bound the size of $\Delta \vh_\ell(\vx)$, let us trust that the first and latter two terms of \cref{eqn:delta_hk} do not cancel (which seems unlikely) and thus observe that
\begin{equation}
    \norm{\Delta \vh_\ell(\vx)}_2
    = \Omega ( \norm{\DW_\ell}_* \cdot \norm{\vh_\ell}_2 )
    = \Omega( \sqrt{d_\ell} ),
\end{equation}
where in the last step we have inserted Condition \ref{cond:scaling}.%
\footnote{This sort of perfect cancellation will be rare in practice, and we can safely ignore it. Adding a small amount of randomness to $\eta_\ell$ will fix any occurrence with high probability.}
Combining this lower bound with our matching upper bound, we conclude that $\norm{\Delta \vh_\ell(\vx)}_2 = \Theta(\sqrt{d_\ell})$ as desired.

We have achieved both clauses of Desideratum \ref{des:scaling} at layer $\ell$, completing the recursive step.
The norm of the input $\vx$ is by assumption the correct size to serve as a base case, and thus we have the correct feature scaling at all layers.

\subsection{Discussion}
We now pause to discuss some key intuitions from the above argument.

\textbf{Weight updates are low-rank and aligned.}
The most important is the observation that, while weight matrices have no special structure at initialization, their subsequent updates are highly structured: they have low rank and align to incoming vectors.
This structure strongly motivates the spectral norm (which describes the action of a matrix on a maximally aligned input) as the correct measure of the size of $\DW_\ell$.

\textbf{Spectral variables enable simpler scaling analysis.}
Most works on hyperparameter scaling discuss parameterwise initialization scales $\sigma_\ell$ and learning rates $\eta_\ell$ as the primary variables.
By contrast, we work directly in terms of the ultimate quantities these hyperparameters regulate: the spectral norms of $\mW_\ell$ and $\DW_\ell$.
This enables us to find the sizes of hidden vectors and their updates quite easily, whereas the same calculation in terms of $\sigma_\ell$ and $\eta_\ell$ is much more involved.%
\footnote{
To see this, note that Equation \ref{eqn:DW} depends not only on $\eta_\ell$ but also --- via the forward signal and backward gradient --- on $\sigma_\ell$ at \textit{every} $\ell \neq \ell$.
}
% It is much easier to just prescribe $\norm{\DW_\ell}_*$ directly.}
% $\vh_\ell(\vx)$ and $\Delta \vh_\ell(\vx)$
We will show how to painlessly recover $\sigma_\ell$ and $\eta_\ell$ from our spectral scaling condition in Section [SECTION].

% let's pause to extract some key intuitions

% it might seem unusual that we have only discussed the sizes of matrices and not the usual DOFs. we will get to how to implement Condition \ref{cond:scaling} in Section [SECTION]. note that the fact that we avoid having to discuss these quantities at all, and this is really the strength of the spectral language here --- since we really care about the sizes of hidden vectors, talking directly about the spectral norms of weight matrices is really the right thing to do.

% probably the most important intuition is that weight-matrix updates are low-rank and align with incoming vectors.



% introduce claims
% make claims
% use claims
% only have to discuss one term


% We will first argue that the features $\vh_\ell(\vx)$ and their change $\Delta \vh(\vx)$ are not too large under \cref{cond:scaling}. Applying the triangle inequality and the operator norm bound to the above recursive expressions, we obtain:
% \begin{align*}
%     \norm{\vh_{\ell}(\vx)}_2 &\leq \norm{\mW_\ell}_* \norm{\vh_{\ell-1}(\vx)}_2; \\
%     \norm{\Delta \vh_\ell(\vx)}_2 &\leq \norm{\Delta \mW_\ell}_* \norm{\vh_{\ell-1}(\vx)}_2 + \norm{\mW_\ell}_* \norm{\Delta \vh_{\ell-1}(\vx)}_2 + \norm{\Delta \mW_\ell}_* \norm{\Delta \vh_{\ell-1}(\vx)}_2.
% \end{align*}

% Under desideratum and condition, this implies what we want. Next, we need to argue that the features and the change in features aren't \textit{too small}. This follows from the following claims:

% \begin{claim}\label{fact:random}
% Fix a feature vector $\vh_{\ell-1}(\vx)\in\R^{d_{\ell-1}}$ and sample a weight matrix $\mW_\ell$ in $\R^{d_\ell\times d_{\ell-1}}$ using a common weight initialisation strategy. Provided that $d_\ell \geq d_{\ell-1}$, then with high probability:
%     \begin{equation*}
%     \norm{ \mW_{\ell}\vh_{\ell-1}(\vx)}_2 = \Theta (\norm{\mW_{\ell}}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2).
%     \end{equation*}
% \end{claim}
% \begin{claim}\label{fact:update} For a matrix $\Delta \mW_\ell$ given by gradient descent at batch size 1.
%     \begin{equation*}\norm{ \Delta\mW_{\ell}\vh_{\ell-1}(\vx)}_2 = \norm{\Delta\mW_{\ell}}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2.
%     \end{equation*}
% \end{claim}
% observe that a gradient descent update is given by: $\Delta \mW_\ell = -\eta \cdot \nabla_{\vh_{\ell}(\vx)}\el \cdot \vh_{\ell-1}(\vx)^\top$ where $\eta$ denotes the learning rate. Then:
% \begin{align*}
%     \norm{\Delta\mW_{\ell}\vh_{\ell-1}(\vx)}_2 &= \norm{-\eta \cdot \nabla_{\vh_{\ell}(\vx)}\el \cdot \norm{\vh_{\ell-1}(\vx)}_2^2}_2 = \eta \norm{\nabla_{\vh_{\ell}(\vx)}\el}_2 \cdot \norm{\vh_{\ell-1}(\vx)}_2^2 = \norm{\Delta \mW_\ell}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2.
% \end{align*}

% \section{Extensions}

% \paragraph{Extension to further gradient steps}

% \paragraph{Extension to larger batch size}

% \paragraph{Extension to nonlinear network}

% \paragraph{Extension to other architectures}

% \begin{enumerate}
%     \item introduction
%     \item preliminaries
%     \item quick derivation
%     \item extensions
%     \item tables + experiments about effective rank
%     \item recover muP, NTP and fact that Delta W doesn't vanish in spectral norm, Frobenius updates
%     \item behaviour at last layer
%     \item related work
%     \item conclusion
% \end{enumerate}

==> old_sections/short-derivation.tex <==
\section{Quick derivation}

To reiterate, we desire that the features at the $\ell$th layer $\vh_\ell(\vx)\in\R^{d_\ell}$ should scale like $\norm{\vh_\ell(\vx)}_2 = \Theta(\sqrt{d_\ell})$ at initialisation, and the change in features induced by a gradient step should also satisfy $\norm{\Delta \vh_\ell(\vx)}_2 = \Theta(\sqrt{d_\ell})$. We will provide an informal argument that this is indeed the case under our spectral scaling (\cref{cond:scaling}). We will argue recursively: if the features at the previous layer $\vh_{\ell-1}(\vx)$ are on the right scale, then the features at the next layer $\vh_{\ell}(\vx)$ will be on the right scale too.

First, it will help to write out recursive expressions for the features and their change after a step:
\begin{align*}
    \vh_{\ell}(\vx) &= \mW_\ell \vh_{\ell-1}(\vx); \\
    \Delta \vh_\ell(\vx) &= \Delta \mW_\ell \vh_{\ell-1}(\vx) + \mW_\ell \Delta \vh_{\ell-1}(\vx) + \Delta \mW_\ell \Delta \vh_{\ell-1}(\vx).
\end{align*}

We will first argue that the features $\vh_\ell(\vx)$ and their change $\Delta \vh(\vx)$ are not too large under \cref{cond:scaling}. Applying the triangle inequality and the operator norm bound to the above recursive expressions, we obtain:
\begin{align*}
    \norm{\vh_{\ell}(\vx)}_2 &\leq \norm{\mW_\ell}_* \norm{\vh_{\ell-1}(\vx)}_2; \\
    \norm{\Delta \vh_\ell(\vx)}_2 &\leq \norm{\Delta \mW_\ell}_* \norm{\vh_{\ell-1}(\vx)}_2 + \norm{\mW_\ell}_* \norm{\Delta \vh_{\ell-1}(\vx)}_2 + \norm{\Delta \mW_\ell}_* \norm{\Delta \vh_{\ell-1}(\vx)}_2.
\end{align*}

Under desideratum and condition, this implies what we want. Next, we need to argue that the features and the change in features aren't \textit{too small}. This follows from the following claims:

\begin{claim}\label{fact:random}
Fix a feature vector $\vh_{\ell-1}(\vx)\in\R^{d_{\ell-1}}$ and sample a weight matrix $\mW_\ell$ in $\R^{d_\ell\times d_{\ell-1}}$ using a common weight initialisation strategy. Provided that $d_\ell \geq d_{\ell-1}$, then with high probability:
    \begin{equation*}
    \norm{ \mW_{\ell}\vh_{\ell-1}(\vx)}_2 = \Theta (\norm{\mW_{\ell}}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2).
    \end{equation*}
\end{claim}
\begin{claim}\label{fact:update} For a matrix $\Delta \mW_\ell$ given by gradient descent at batch size 1.
    \begin{equation*}\norm{ \Delta\mW_{\ell}\vh_{\ell-1}(\vx)}_2 = \norm{\Delta\mW_{\ell}}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2.
    \end{equation*}
\end{claim}
observe that a gradient descent update is given by: $\Delta \mW_\ell = -\eta \cdot \nabla_{\vh_{\ell}(\vx)}\el \cdot \vh_{\ell-1}(\vx)^\top$ where $\eta$ denotes the learning rate. Then:
\begin{align*}
    \norm{\Delta\mW_{\ell}\vh_{\ell-1}(\vx)}_2 &= \norm{-\eta \cdot \nabla_{\vh_{\ell}(\vx)}\el \cdot \norm{\vh_{\ell-1}(\vx)}_2^2}_2 = \eta \norm{\nabla_{\vh_{\ell}(\vx)}\el}_2 \cdot \norm{\vh_{\ell-1}(\vx)}_2^2 = \norm{\Delta \mW_\ell}_* \cdot \norm{\vh_{\ell-1}(\vx)}_2.
\end{align*}

\section{Extensions}

\paragraph{Extension to further gradient steps}

\paragraph{Extension to larger batch size}

\paragraph{Extension to nonlinear network}

\paragraph{Extension to other architectures}

\begin{enumerate}
    \item introduction
    \item preliminaries
    \item quick derivation
    \item extensions
    \item tables + experiments about effective rank
    \item recover muP, NTP and fact that Delta W doesn't vanish in spectral norm, Frobenius updates
    \item behaviour at last layer
    \item related work
    \item conclusion
\end{enumerate}

==> table/init.tex <==
\renewcommand{\arraystretch}{3.0}
\begin{table}
    \centering
    \begin{tabular}{| c | c | c |}
     \hline
     Random initializer for $\mW_\ell^\prime$& Dimension & Multiplier $\alpha$ for $\mW_\ell = \alpha \times \mW_\ell^\prime$\\[1ex]
     \hline\hline
     standard Normal & $d_\ell\times d_{\ell-1}$ & $\displaystyle\frac{1}{\sqrt{d_{\ell}} + \sqrt{d_{\ell-1}}} \times \sqrt{\frac{d_{\ell}}{d_{\ell-1}}}$ \\[1ex]
     \hline
     uniform semi-orthogonal & $d_\ell\times d_{\ell-1}$ & $\displaystyle
 \sqrt{\frac{d_\ell}{d_{\ell-1}}}$ \\[1ex]
     \hline
    \end{tabular}
    \caption{Satisfying the spectral scaling condition (\cref{cond:scaling}) at initialization. We consider drawing a temporary matrix $\mW^\prime_\ell$ using a standard weight initializer, and then re-scaling to obtain $\mW_\ell=\alpha \times\mW^\prime_\ell$. This table gives values of $\alpha$ for common weight initializers such that $\smash{\norm{\mW_\ell}_* \approx \sqrt{d_\ell / d_{\ell-1}}}$.}
    \label{tab:init}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> table/update.tex <==
\renewcommand{\arraystretch}{3.0}
\begin{table}
    \centering
    \begin{tabular}{| c | c c | c c c|}
     \hline
     Matrix & Dimension & Stable rank & Spectral norm & Frobenius proxy & Norm-free proxy \\[1ex]
     \hline\hline
     $\mW_\ell$ & $d_\ell\times d_{\ell-1}$ & $\min(d_\ell,d_{\ell-1})$ & $\displaystyle\norm{\mW_\ell}_*$ & $\displaystyle\frac{\norm{\mW_\ell}_F}{\sqrt{\min(d_\ell,d_{\ell-1})}}$ & $\displaystyle\sqrt{\frac{d_\ell}{d_{\ell-1}}}$ \\[1ex]
     \hline
     $\nabla_{\mW_\ell}\mathcal{L}$ & $d_\ell\times d_{\ell-1}$ & $1$ & $\displaystyle\norm{\nabla_{\mW_\ell}\mathcal{L}}_*$ & $\displaystyle\norm{\nabla_{\mW_\ell}\mathcal{L}}_F$ & $\displaystyle\sqrt{\frac{d_{\ell-1}}{d_{\ell}}}$ \\[1ex]
     \hline
    \end{tabular}
    \caption[]{Cheap proxies for the spectral norm. Consider making a gradient update $\DW_\ell$ to the $\ell$th weight matrix $\mW_\ell$ in a multilayer perceptron. To satisfy \cref{cond:scaling}, the update should be scaled:
    \begin{equation*}
        \DW_\ell = - \eta \times \frac{\norm{\mW_\ell}_*}{\norm{\nabla_{\mW_\ell}\mathcal{L}}_*} \times \nabla_{\mW_\ell}\mathcal{L} \implies \norm{\DW_\ell}_* = \eta \times \norm{\mW_\ell}_*
    \end{equation*}
    where $\eta>0$ is a width-independent learning rate. Since computing the spectral norms $\norm{\mW_\ell}_*$ and $\norm{\nabla_{\mW_\ell}\mathcal{L}}_*$ can be expensive, this table provides more computationally efficient substitutes.
    }
    \label{tab:conversion}
\end{table}
\renewcommand{\arraystretch}{1.0}
